A Residuals-Based Nonparametric Variance Ratio Test for Cointegration

This paper derives asymptotic theory for Breitung's (2002, Journal of Econometrics 108, 343-363) nonparameteric variance ratio unit root test when applied to regression residuals. The test requires neither the specification of the correlation structure in the data nor the choice of tuning parameters. Compared with popular residuals-based no-cointegration tests, the variance ratio test is less prone to size distortions but has smaller local asymptotic power. However, this paper shows that local asymptotic power properties do not serve as a useful indicator for the power of residuals-based no-cointegration tests in finite samples. In terms of size-corrected power, the variance ratio test performs relatively well and, in particular, does not suffer from power reversal problems detected for, e.g., the frequently used augmented Dickey-Fuller type no-cointegration test. An application to daily prices of cryptocurrencies illustrates the usefulness of the variance ratio test in practice.

==> Figures/Empirical_Sizes/2022-07-14/Size_table_m_1_T_100_dtype0_AIC.tex <==

\begin{table}[!ht]
\begin{center}
\caption{Size-table-m-1-T-100-dtype0-AIC}
\begin{tabular}{c|cccccccccccc}
\hline
&$\rho_1,\rho_2$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\\hline
&$\text{VR}$ & 0.02 & 0.01 & 0.01 & 0.01 & 0.02 & 0.03 & 0.17 & 0.02 & 0.02 & 0.01 & 0.02 & 0.02 \\
&$\text{VR}^{(\GLS)}$ & 0.02 & 0.01 & 0.01 & 0.01 & 0.02 & 0.03 & 0.17 & 0.02 & 0.02 & 0.01 & 0.02 & 0.02 \\
&ADF & 0.08 & 0.07 & 0.07 & 0.06 & 0.10 & 0.14 & 0.43 & 0.14 & 0.08 & 0.07 & 0.08 & 0.08 \\
&$\text{ADF}^{(\GLS)}$ & 0.08 & 0.07 & 0.07 & 0.06 & 0.10 & 0.14 & 0.43 & 0.14 & 0.08 & 0.07 & 0.08 & 0.08 \\
&$\text{ADF}^*$ & 0.05 & 0.04 & 0.04 & 0.04 & 0.06 & 0.06 & 0.14 & 0.07 & 0.05 & 0.04 & 0.05 & 0.05 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.04 & 0.04 & 0.04 & 0.06 & 0.06 & 0.14 & 0.07 & 0.05 & 0.04 & 0.05 & 0.05 \\
&MSB & 0.04 & 0.04 & 0.04 & 0.05 & 0.05 & 0.07 & 0.33 & 0.07 & 0.04 & 0.04 & 0.04 & 0.04 \\
&$\text{MSB}^{(\GLS)*}$ & 0.01 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.07 & 0.02 & 0.01 & 0.00 & 0.01 & 0.01 \\
&$\hat{Z}_{\alpha}$ & 0.03 & 0.02 & 0.01 & 0.01 & 0.07 & 0.30 & 0.89 & 0.13 & 0.03 & 0.01 & 0.03 & 0.03 \\
&$\text{VR}$ & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.03 & 0.17 & 0.02 & 0.01 & 0.01 & 0.01 & 0.01 \\
&$\text{VR}^{(\GLS)}$ & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.03 & 0.17 & 0.02 & 0.01 & 0.01 & 0.01 & 0.01 \\
&ADF & 0.07 & 0.08 & 0.07 & 0.07 & 0.10 & 0.13 & 0.45 & 0.13 & 0.07 & 0.07 & 0.07 & 0.07 \\
&$\text{ADF}^{(\GLS)}$ & 0.07 & 0.08 & 0.07 & 0.07 & 0.10 & 0.13 & 0.45 & 0.13 & 0.07 & 0.07 & 0.07 & 0.07 \\
&$\text{ADF}^*$ & 0.05 & 0.04 & 0.05 & 0.05 & 0.06 & 0.06 & 0.15 & 0.07 & 0.05 & 0.05 & 0.05 & 0.05 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.04 & 0.05 & 0.05 & 0.06 & 0.06 & 0.15 & 0.07 & 0.05 & 0.05 & 0.05 & 0.05 \\
&MSB & 0.03 & 0.04 & 0.04 & 0.04 & 0.04 & 0.07 & 0.34 & 0.07 & 0.03 & 0.04 & 0.03 & 0.03 \\
&$\text{MSB}^{(\GLS)*}$ & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.08 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 \\
&$\hat{Z}_{\alpha}$ & 0.02 & 0.02 & 0.02 & 0.02 & 0.07 & 0.31 & 0.89 & 0.12 & 0.03 & 0.02 & 0.02 & 0.02 \\
&$\text{VR}$ & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.03 & 0.18 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 \\
&$\text{VR}^{(\GLS)}$ & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.03 & 0.18 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 \\
&ADF & 0.08 & 0.08 & 0.10 & 0.09 & 0.09 & 0.14 & 0.47 & 0.13 & 0.07 & 0.08 & 0.08 & 0.07 \\
&$\text{ADF}^{(\GLS)}$ & 0.08 & 0.08 & 0.10 & 0.09 & 0.09 & 0.14 & 0.47 & 0.13 & 0.07 & 0.08 & 0.08 & 0.07 \\
&$\text{ADF}^*$ & 0.05 & 0.06 & 0.07 & 0.06 & 0.06 & 0.06 & 0.17 & 0.07 & 0.05 & 0.05 & 0.05 & 0.05 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.06 & 0.07 & 0.06 & 0.06 & 0.06 & 0.17 & 0.07 & 0.05 & 0.05 & 0.05 & 0.05 \\
&MSB & 0.02 & 0.03 & 0.03 & 0.04 & 0.03 & 0.07 & 0.37 & 0.06 & 0.02 & 0.03 & 0.02 & 0.02 \\
&$\text{MSB}^{(\GLS)*}$ & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.09 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\
&$\hat{Z}_{\alpha}$ & 0.02 & 0.02 & 0.04 & 0.03 & 0.07 & 0.34 & 0.89 & 0.13 & 0.02 & 0.02 & 0.02 & 0.02 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> Figures/Empirical_Sizes/2022-07-14/Size_table_m_1_T_100_dtype1_AIC.tex <==

\begin{table}[!ht]
\begin{center}
\caption{Size-table-m-1-T-100-dtype1-AIC}
\begin{tabular}{c|cccccccccccc}
\hline
&$\rho_1,\rho_2$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\\hline
&$\text{VR}$ & 0.05 & 0.04 & 0.03 & 0.01 & 0.07 & 0.16 & 0.72 & 0.10 & 0.05 & 0.03 & 0.05 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.12 & 0.11 & 0.08 & 0.03 & 0.15 & 0.26 & 0.82 & 0.19 & 0.12 & 0.09 & 0.12 & 0.12 \\
&ADF & 0.08 & 0.07 & 0.07 & 0.05 & 0.13 & 0.23 & 0.83 & 0.24 & 0.08 & 0.06 & 0.09 & 0.08 \\
&$\text{ADF}^{(\GLS)}$ & 0.11 & 0.10 & 0.09 & 0.06 & 0.17 & 0.26 & 0.70 & 0.28 & 0.11 & 0.09 & 0.11 & 0.11 \\
&$\text{ADF}^*$ & 0.04 & 0.02 & 0.02 & 0.02 & 0.05 & 0.07 & 0.34 & 0.08 & 0.04 & 0.01 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.06 & 0.03 & 0.03 & 0.01 & 0.08 & 0.10 & 0.37 & 0.12 & 0.06 & 0.02 & 0.06 & 0.06 \\
&MSB & 0.11 & 0.14 & 0.14 & 0.15 & 0.14 & 0.21 & 0.77 & 0.22 & 0.11 & 0.14 & 0.12 & 0.11 \\
&$\text{MSB}^{(\GLS)*}$ & 0.02 & 0.02 & 0.03 & 0.03 & 0.04 & 0.05 & 0.27 & 0.08 & 0.02 & 0.01 & 0.03 & 0.02 \\
&$\hat{Z}_{\alpha}$ & 0.05 & 0.02 & 0.01 & 0.01 & 0.19 & 0.72 & 1.00 & 0.33 & 0.05 & 0.01 & 0.05 & 0.05 \\
&$\text{VR}$ & 0.05 & 0.04 & 0.03 & 0.01 & 0.07 & 0.19 & 0.78 & 0.11 & 0.05 & 0.03 & 0.05 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.12 & 0.11 & 0.09 & 0.05 & 0.16 & 0.29 & 0.85 & 0.20 & 0.12 & 0.09 & 0.12 & 0.12 \\
&ADF & 0.08 & 0.08 & 0.08 & 0.05 & 0.14 & 0.28 & 0.87 & 0.26 & 0.08 & 0.07 & 0.09 & 0.08 \\
&$\text{ADF}^{(\GLS)}$ & 0.11 & 0.11 & 0.10 & 0.07 & 0.17 & 0.29 & 0.75 & 0.28 & 0.11 & 0.09 & 0.11 & 0.11 \\
&$\text{ADF}^*$ & 0.04 & 0.02 & 0.03 & 0.02 & 0.05 & 0.07 & 0.38 & 0.08 & 0.04 & 0.02 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.06 & 0.03 & 0.03 & 0.02 & 0.08 & 0.10 & 0.42 & 0.12 & 0.06 & 0.03 & 0.06 & 0.06 \\
&MSB & 0.12 & 0.14 & 0.14 & 0.14 & 0.14 & 0.24 & 0.82 & 0.25 & 0.12 & 0.14 & 0.12 & 0.12 \\
&$\text{MSB}^{(\GLS)*}$ & 0.03 & 0.02 & 0.03 & 0.03 & 0.04 & 0.05 & 0.30 & 0.08 & 0.03 & 0.02 & 0.03 & 0.03 \\
&$\hat{Z}_{\alpha}$ & 0.06 & 0.03 & 0.03 & 0.02 & 0.21 & 0.79 & 1.00 & 0.39 & 0.06 & 0.02 & 0.06 & 0.06 \\
&$\text{VR}$ & 0.05 & 0.05 & 0.06 & 0.01 & 0.09 & 0.31 & 0.87 & 0.15 & 0.05 & 0.05 & 0.05 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.12 & 0.12 & 0.14 & 0.06 & 0.18 & 0.43 & 0.93 & 0.26 & 0.12 & 0.12 & 0.12 & 0.12 \\
&ADF & 0.08 & 0.10 & 0.16 & 0.06 & 0.15 & 0.41 & 0.92 & 0.33 & 0.08 & 0.11 & 0.10 & 0.08 \\
&$\text{ADF}^{(\GLS)}$ & 0.11 & 0.13 & 0.20 & 0.10 & 0.19 & 0.40 & 0.79 & 0.35 & 0.11 & 0.15 & 0.12 & 0.11 \\
&$\text{ADF}^*$ & 0.04 & 0.04 & 0.07 & 0.03 & 0.05 & 0.10 & 0.45 & 0.10 & 0.04 & 0.05 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.06 & 0.06 & 0.11 & 0.05 & 0.08 & 0.14 & 0.48 & 0.14 & 0.06 & 0.07 & 0.06 & 0.06 \\
&MSB & 0.11 & 0.13 & 0.16 & 0.12 & 0.16 & 0.35 & 0.89 & 0.32 & 0.11 & 0.14 & 0.12 & 0.12 \\
&$\text{MSB}^{(\GLS)*}$ & 0.03 & 0.03 & 0.06 & 0.03 & 0.04 & 0.06 & 0.36 & 0.09 & 0.03 & 0.04 & 0.03 & 0.03 \\
&$\hat{Z}_{\alpha}$ & 0.06 & 0.07 & 0.14 & 0.04 & 0.36 & 0.95 & 1.00 & 0.59 & 0.06 & 0.08 & 0.06 & 0.06 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> Figures/Empirical_Sizes/2022-07-14/Size_table_m_1_T_100_dtype2_AIC.tex <==

\begin{table}[!ht]
\begin{center}
\caption{Size-table-m-1-T-100-dtype2-AIC}
\begin{tabular}{c|cccccccccccc}
\hline
&$\rho_1,\rho_2$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\\hline
&$\text{VR}$ & 0.05 & 0.04 & 0.02 & 0.00 & 0.09 & 0.26 & 0.93 & 0.14 & 0.05 & 0.03 & 0.06 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.30 & 0.26 & 0.20 & 0.07 & 0.36 & 0.59 & 0.99 & 0.45 & 0.30 & 0.22 & 0.30 & 0.30 \\
&ADF & 0.10 & 0.10 & 0.08 & 0.05 & 0.19 & 0.35 & 0.91 & 0.35 & 0.10 & 0.08 & 0.10 & 0.10 \\
&$\text{ADF}^{(\GLS)}$ & 0.14 & 0.13 & 0.12 & 0.07 & 0.23 & 0.37 & 0.85 & 0.39 & 0.14 & 0.11 & 0.14 & 0.14 \\
&$\text{ADF}^*$ & 0.03 & 0.01 & 0.02 & 0.01 & 0.06 & 0.09 & 0.51 & 0.11 & 0.03 & 0.01 & 0.04 & 0.03 \\
&$\text{ADF}^{(\GLS)*}$ & 0.06 & 0.02 & 0.03 & 0.01 & 0.08 & 0.12 & 0.54 & 0.15 & 0.06 & 0.01 & 0.06 & 0.06 \\
&MSB & 0.15 & 0.20 & 0.22 & 0.25 & 0.19 & 0.28 & 0.85 & 0.27 & 0.15 & 0.22 & 0.17 & 0.15 \\
&$\text{MSB}^{(\GLS)*}$ & 0.01 & 0.01 & 0.03 & 0.03 & 0.04 & 0.06 & 0.42 & 0.09 & 0.01 & 0.01 & 0.02 & 0.01 \\
&$\hat{Z}_{\alpha}$ & 0.04 & 0.01 & 0.00 & 0.00 & 0.24 & 0.87 & 1.00 & 0.43 & 0.04 & 0.00 & 0.05 & 0.04 \\
&$\text{VR}$ & 0.05 & 0.04 & 0.03 & 0.00 & 0.09 & 0.30 & 0.94 & 0.15 & 0.05 & 0.03 & 0.05 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.30 & 0.26 & 0.22 & 0.08 & 0.38 & 0.64 & 0.99 & 0.47 & 0.30 & 0.23 & 0.30 & 0.30 \\
&ADF & 0.11 & 0.10 & 0.09 & 0.05 & 0.20 & 0.40 & 0.92 & 0.38 & 0.11 & 0.09 & 0.11 & 0.11 \\
&$\text{ADF}^{(\GLS)}$ & 0.14 & 0.13 & 0.11 & 0.08 & 0.23 & 0.41 & 0.86 & 0.41 & 0.14 & 0.11 & 0.14 & 0.14 \\
&$\text{ADF}^*$ & 0.04 & 0.01 & 0.02 & 0.01 & 0.06 & 0.10 & 0.48 & 0.11 & 0.04 & 0.01 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.06 & 0.02 & 0.03 & 0.01 & 0.09 & 0.14 & 0.51 & 0.16 & 0.06 & 0.01 & 0.06 & 0.06 \\
&MSB & 0.16 & 0.19 & 0.20 & 0.23 & 0.19 & 0.33 & 0.86 & 0.30 & 0.16 & 0.21 & 0.17 & 0.16 \\
&$\text{MSB}^{(\GLS)*}$ & 0.02 & 0.01 & 0.02 & 0.03 & 0.04 & 0.07 & 0.39 & 0.10 & 0.02 & 0.01 & 0.02 & 0.02 \\
&$\hat{Z}_{\alpha}$ & 0.04 & 0.01 & 0.01 & 0.00 & 0.28 & 0.93 & 1.00 & 0.48 & 0.04 & 0.01 & 0.05 & 0.05 \\
&$\text{VR}$ & 0.05 & 0.05 & 0.06 & 0.00 & 0.11 & 0.48 & 0.98 & 0.20 & 0.05 & 0.04 & 0.05 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.29 & 0.29 & 0.32 & 0.09 & 0.43 & 0.81 & 1.00 & 0.56 & 0.29 & 0.28 & 0.30 & 0.29 \\
&ADF & 0.11 & 0.11 & 0.15 & 0.04 & 0.22 & 0.57 & 0.93 & 0.47 & 0.11 & 0.11 & 0.11 & 0.11 \\
&$\text{ADF}^{(\GLS)}$ & 0.13 & 0.15 & 0.20 & 0.06 & 0.25 & 0.55 & 0.86 & 0.48 & 0.13 & 0.15 & 0.14 & 0.14 \\
&$\text{ADF}^*$ & 0.04 & 0.03 & 0.05 & 0.01 & 0.06 & 0.14 & 0.45 & 0.14 & 0.04 & 0.03 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.06 & 0.05 & 0.08 & 0.01 & 0.09 & 0.18 & 0.48 & 0.18 & 0.06 & 0.05 & 0.06 & 0.06 \\
&MSB & 0.16 & 0.17 & 0.17 & 0.17 & 0.21 & 0.48 & 0.88 & 0.41 & 0.16 & 0.17 & 0.17 & 0.16 \\
&$\text{MSB}^{(\GLS)*}$ & 0.02 & 0.02 & 0.03 & 0.01 & 0.04 & 0.10 & 0.36 & 0.12 & 0.02 & 0.01 & 0.02 & 0.02 \\
&$\hat{Z}_{\alpha}$ & 0.05 & 0.05 & 0.09 & 0.00 & 0.46 & 1.00 & 1.00 & 0.70 & 0.05 & 0.05 & 0.05 & 0.05 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> Figures/Empirical_Sizes/2022-07-14/Size_table_m_1_T_250_dtype0_AIC.tex <==

\begin{table}[!ht]
\begin{center}
\caption{Size-table-m-1-T-250-dtype0-AIC}
\begin{tabular}{c|cccccccccccc}
\hline
&$\rho_1,\rho_2$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\\hline
&$\text{VR}$ & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 & 0.03 & 0.14 & 0.03 & 0.02 & 0.02 & 0.02 & 0.02 \\
&$\text{VR}^{(\GLS)}$ & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 & 0.03 & 0.14 & 0.03 & 0.02 & 0.02 & 0.02 & 0.02 \\
&ADF & 0.06 & 0.06 & 0.05 & 0.04 & 0.07 & 0.09 & 0.32 & 0.09 & 0.06 & 0.05 & 0.06 & 0.06 \\
&$\text{ADF}^{(\GLS)}$ & 0.06 & 0.06 & 0.05 & 0.04 & 0.07 & 0.09 & 0.32 & 0.09 & 0.06 & 0.05 & 0.06 & 0.06 \\
&$\text{ADF}^*$ & 0.04 & 0.04 & 0.03 & 0.03 & 0.05 & 0.05 & 0.11 & 0.05 & 0.04 & 0.03 & 0.05 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.04 & 0.04 & 0.03 & 0.03 & 0.05 & 0.05 & 0.11 & 0.05 & 0.04 & 0.03 & 0.05 & 0.04 \\
&MSB & 0.03 & 0.03 & 0.03 & 0.03 & 0.04 & 0.05 & 0.17 & 0.06 & 0.03 & 0.03 & 0.04 & 0.03 \\
&$\text{MSB}^{(\GLS)*}$ & 0.02 & 0.01 & 0.01 & 0.01 & 0.02 & 0.02 & 0.01 & 0.02 & 0.01 & 0.01 & 0.01 & 0.01 \\
&$\hat{Z}_{\alpha}$ & 0.03 & 0.02 & 0.02 & 0.01 & 0.07 & 0.31 & 0.94 & 0.14 & 0.03 & 0.02 & 0.03 & 0.03 \\
&$\text{VR}$ & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 & 0.03 & 0.16 & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 \\
&$\text{VR}^{(\GLS)}$ & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 & 0.03 & 0.16 & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 \\
&ADF & 0.06 & 0.06 & 0.06 & 0.06 & 0.07 & 0.10 & 0.36 & 0.09 & 0.06 & 0.05 & 0.06 & 0.06 \\
&$\text{ADF}^{(\GLS)}$ & 0.06 & 0.06 & 0.06 & 0.06 & 0.07 & 0.10 & 0.36 & 0.09 & 0.06 & 0.05 & 0.06 & 0.06 \\
&$\text{ADF}^*$ & 0.04 & 0.04 & 0.04 & 0.04 & 0.05 & 0.06 & 0.14 & 0.05 & 0.04 & 0.04 & 0.05 & 0.05 \\
&$\text{ADF}^{(\GLS)*}$ & 0.04 & 0.04 & 0.04 & 0.04 & 0.05 & 0.06 & 0.14 & 0.05 & 0.04 & 0.04 & 0.05 & 0.05 \\
&MSB & 0.02 & 0.03 & 0.03 & 0.03 & 0.03 & 0.04 & 0.21 & 0.05 & 0.03 & 0.03 & 0.03 & 0.03 \\
&$\text{MSB}^{(\GLS)*}$ & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.02 & 0.02 & 0.01 & 0.01 & 0.01 & 0.01 \\
&$\hat{Z}_{\alpha}$ & 0.03 & 0.02 & 0.02 & 0.03 & 0.07 & 0.35 & 0.95 & 0.15 & 0.03 & 0.02 & 0.03 & 0.03 \\
&$\text{VR}$ & 0.01 & 0.01 & 0.01 & 0.02 & 0.02 & 0.03 & 0.18 & 0.02 & 0.01 & 0.01 & 0.01 & 0.01 \\
&$\text{VR}^{(\GLS)}$ & 0.01 & 0.01 & 0.01 & 0.02 & 0.02 & 0.03 & 0.18 & 0.02 & 0.01 & 0.01 & 0.01 & 0.01 \\
&ADF & 0.06 & 0.07 & 0.10 & 0.12 & 0.08 & 0.11 & 0.42 & 0.10 & 0.06 & 0.08 & 0.06 & 0.06 \\
&$\text{ADF}^{(\GLS)}$ & 0.06 & 0.07 & 0.10 & 0.12 & 0.08 & 0.11 & 0.42 & 0.10 & 0.06 & 0.08 & 0.06 & 0.06 \\
&$\text{ADF}^*$ & 0.05 & 0.05 & 0.06 & 0.09 & 0.05 & 0.06 & 0.20 & 0.06 & 0.05 & 0.06 & 0.05 & 0.05 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.05 & 0.06 & 0.09 & 0.05 & 0.06 & 0.20 & 0.06 & 0.05 & 0.06 & 0.05 & 0.05 \\
&MSB & 0.02 & 0.02 & 0.05 & 0.07 & 0.03 & 0.03 & 0.28 & 0.04 & 0.02 & 0.03 & 0.02 & 0.02 \\
&$\text{MSB}^{(\GLS)*}$ & 0.01 & 0.01 & 0.02 & 0.04 & 0.01 & 0.01 & 0.05 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 \\
&$\hat{Z}_{\alpha}$ & 0.02 & 0.03 & 0.08 & 0.09 & 0.08 & 0.43 & 0.96 & 0.18 & 0.02 & 0.04 & 0.03 & 0.02 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> Figures/Empirical_Sizes/2022-07-14/Size_table_m_1_T_250_dtype1_AIC.tex <==

\begin{table}[!ht]
\begin{center}
\caption{Size-table-m-1-T-250-dtype1-AIC}
\begin{tabular}{c|cccccccccccc}
\hline
&$\rho_1,\rho_2$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\\hline
&$\text{VR}$ & 0.05 & 0.05 & 0.04 & 0.02 & 0.06 & 0.10 & 0.56 & 0.08 & 0.05 & 0.04 & 0.06 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.10 & 0.10 & 0.09 & 0.06 & 0.11 & 0.15 & 0.55 & 0.12 & 0.10 & 0.09 & 0.10 & 0.10 \\
&ADF & 0.06 & 0.06 & 0.05 & 0.04 & 0.08 & 0.12 & 0.61 & 0.12 & 0.06 & 0.05 & 0.07 & 0.06 \\
&$\text{ADF}^{(\GLS)}$ & 0.06 & 0.06 & 0.05 & 0.04 & 0.08 & 0.12 & 0.43 & 0.13 & 0.06 & 0.05 & 0.07 & 0.06 \\
&$\text{ADF}^*$ & 0.04 & 0.03 & 0.02 & 0.01 & 0.04 & 0.04 & 0.16 & 0.05 & 0.04 & 0.02 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.04 & 0.04 & 0.03 & 0.01 & 0.05 & 0.05 & 0.16 & 0.06 & 0.04 & 0.02 & 0.04 & 0.04 \\
&MSB & 0.07 & 0.08 & 0.08 & 0.08 & 0.09 & 0.11 & 0.48 & 0.14 & 0.07 & 0.08 & 0.08 & 0.07 \\
&$\text{MSB}^{(\GLS)*}$ & 0.03 & 0.03 & 0.03 & 0.02 & 0.04 & 0.03 & 0.04 & 0.05 & 0.03 & 0.02 & 0.04 & 0.03 \\
&$\hat{Z}_{\alpha}$ & 0.06 & 0.03 & 0.02 & 0.00 & 0.15 & 0.64 & 1.00 & 0.31 & 0.06 & 0.02 & 0.06 & 0.06 \\
&$\text{VR}$ & 0.05 & 0.05 & 0.05 & 0.03 & 0.06 & 0.12 & 0.66 & 0.08 & 0.05 & 0.05 & 0.06 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.10 & 0.10 & 0.10 & 0.07 & 0.12 & 0.17 & 0.62 & 0.13 & 0.10 & 0.10 & 0.11 & 0.10 \\
&ADF & 0.06 & 0.06 & 0.06 & 0.05 & 0.08 & 0.14 & 0.71 & 0.14 & 0.06 & 0.05 & 0.07 & 0.06 \\
&$\text{ADF}^{(\GLS)}$ & 0.07 & 0.07 & 0.07 & 0.06 & 0.09 & 0.14 & 0.49 & 0.14 & 0.07 & 0.06 & 0.08 & 0.07 \\
&$\text{ADF}^*$ & 0.04 & 0.03 & 0.03 & 0.03 & 0.04 & 0.05 & 0.22 & 0.05 & 0.04 & 0.03 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.04 & 0.04 & 0.03 & 0.05 & 0.06 & 0.22 & 0.06 & 0.05 & 0.03 & 0.04 & 0.05 \\
&MSB & 0.07 & 0.08 & 0.09 & 0.08 & 0.10 & 0.12 & 0.60 & 0.15 & 0.07 & 0.08 & 0.09 & 0.07 \\
&$\text{MSB}^{(\GLS)*}$ & 0.04 & 0.04 & 0.04 & 0.03 & 0.05 & 0.03 & 0.07 & 0.05 & 0.04 & 0.03 & 0.03 & 0.03 \\
&$\hat{Z}_{\alpha}$ & 0.06 & 0.04 & 0.04 & 0.03 & 0.18 & 0.74 & 1.00 & 0.36 & 0.06 & 0.03 & 0.06 & 0.06 \\
&$\text{VR}$ & 0.05 & 0.05 & 0.06 & 0.06 & 0.07 & 0.19 & 0.83 & 0.10 & 0.05 & 0.06 & 0.06 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.10 & 0.10 & 0.11 & 0.12 & 0.12 & 0.25 & 0.74 & 0.15 & 0.10 & 0.10 & 0.10 & 0.10 \\
&ADF & 0.06 & 0.07 & 0.14 & 0.13 & 0.09 & 0.21 & 0.89 & 0.17 & 0.06 & 0.09 & 0.07 & 0.06 \\
&$\text{ADF}^{(\GLS)}$ & 0.07 & 0.08 & 0.15 & 0.18 & 0.10 & 0.20 & 0.61 & 0.17 & 0.07 & 0.10 & 0.08 & 0.07 \\
&$\text{ADF}^*$ & 0.04 & 0.04 & 0.06 & 0.08 & 0.04 & 0.05 & 0.41 & 0.06 & 0.04 & 0.04 & 0.04 & 0.03 \\
&$\text{ADF}^{(\GLS)*}$ & 0.04 & 0.05 & 0.08 & 0.12 & 0.05 & 0.07 & 0.39 & 0.07 & 0.04 & 0.06 & 0.04 & 0.04 \\
&MSB & 0.07 & 0.09 & 0.16 & 0.17 & 0.10 & 0.15 & 0.83 & 0.18 & 0.07 & 0.11 & 0.09 & 0.07 \\
&$\text{MSB}^{(\GLS)*}$ & 0.03 & 0.04 & 0.07 & 0.11 & 0.04 & 0.02 & 0.18 & 0.05 & 0.03 & 0.05 & 0.04 & 0.03 \\
&$\hat{Z}_{\alpha}$ & 0.06 & 0.08 & 0.19 & 0.16 & 0.29 & 0.94 & 1.00 & 0.57 & 0.06 & 0.10 & 0.06 & 0.06 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> Figures/Empirical_Sizes/2022-07-14/Size_table_m_1_T_250_dtype2_AIC.tex <==

\begin{table}[!ht]
\begin{center}
\caption{Size-table-m-1-T-250-dtype2-AIC}
\begin{tabular}{c|cccccccccccc}
\hline
&$\rho_1,\rho_2$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\\hline
&$\text{VR}$ & 0.05 & 0.05 & 0.03 & 0.01 & 0.07 & 0.15 & 0.83 & 0.10 & 0.05 & 0.04 & 0.06 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.13 & 0.12 & 0.11 & 0.05 & 0.15 & 0.23 & 0.65 & 0.18 & 0.13 & 0.11 & 0.14 & 0.13 \\
&ADF & 0.07 & 0.07 & 0.06 & 0.04 & 0.10 & 0.18 & 0.79 & 0.19 & 0.07 & 0.06 & 0.08 & 0.07 \\
&$\text{ADF}^{(\GLS)}$ & 0.08 & 0.08 & 0.07 & 0.05 & 0.11 & 0.18 & 0.62 & 0.19 & 0.08 & 0.07 & 0.09 & 0.08 \\
&$\text{ADF}^*$ & 0.04 & 0.03 & 0.03 & 0.01 & 0.04 & 0.05 & 0.24 & 0.06 & 0.04 & 0.01 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.04 & 0.03 & 0.01 & 0.06 & 0.07 & 0.25 & 0.07 & 0.05 & 0.02 & 0.04 & 0.04 \\
&MSB & 0.09 & 0.11 & 0.12 & 0.14 & 0.12 & 0.15 & 0.68 & 0.19 & 0.09 & 0.12 & 0.10 & 0.09 \\
&$\text{MSB}^{(\GLS)*}$ & 0.03 & 0.04 & 0.03 & 0.03 & 0.05 & 0.03 & 0.11 & 0.06 & 0.03 & 0.01 & 0.03 & 0.03 \\
&$\hat{Z}_{\alpha}$ & 0.05 & 0.03 & 0.01 & 0.00 & 0.21 & 0.83 & 1.00 & 0.43 & 0.05 & 0.01 & 0.06 & 0.06 \\
&$\text{VR}$ & 0.05 & 0.05 & 0.04 & 0.01 & 0.07 & 0.19 & 0.91 & 0.10 & 0.05 & 0.04 & 0.05 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.13 & 0.12 & 0.11 & 0.07 & 0.15 & 0.25 & 0.69 & 0.19 & 0.13 & 0.11 & 0.13 & 0.13 \\
&ADF & 0.08 & 0.08 & 0.07 & 0.05 & 0.11 & 0.20 & 0.87 & 0.19 & 0.08 & 0.06 & 0.09 & 0.08 \\
&$\text{ADF}^{(\GLS)}$ & 0.08 & 0.08 & 0.08 & 0.06 & 0.12 & 0.21 & 0.68 & 0.20 & 0.08 & 0.07 & 0.09 & 0.09 \\
&$\text{ADF}^*$ & 0.04 & 0.03 & 0.03 & 0.02 & 0.04 & 0.05 & 0.29 & 0.06 & 0.04 & 0.02 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.04 & 0.03 & 0.02 & 0.06 & 0.06 & 0.29 & 0.08 & 0.05 & 0.02 & 0.05 & 0.05 \\
&MSB & 0.08 & 0.11 & 0.11 & 0.11 & 0.12 & 0.16 & 0.79 & 0.20 & 0.08 & 0.11 & 0.11 & 0.09 \\
&$\text{MSB}^{(\GLS)*}$ & 0.03 & 0.03 & 0.03 & 0.02 & 0.04 & 0.03 & 0.15 & 0.06 & 0.03 & 0.02 & 0.03 & 0.03 \\
&$\hat{Z}_{\alpha}$ & 0.06 & 0.03 & 0.03 & 0.01 & 0.25 & 0.91 & 1.00 & 0.51 & 0.06 & 0.02 & 0.06 & 0.06 \\
&$\text{VR}$ & 0.05 & 0.06 & 0.07 & 0.03 & 0.09 & 0.32 & 0.99 & 0.15 & 0.05 & 0.06 & 0.05 & 0.06 \\
&$\text{VR}^{(\GLS)}$ & 0.13 & 0.13 & 0.15 & 0.13 & 0.16 & 0.35 & 0.73 & 0.22 & 0.13 & 0.13 & 0.13 & 0.13 \\
&ADF & 0.07 & 0.09 & 0.18 & 0.09 & 0.12 & 0.32 & 0.96 & 0.25 & 0.07 & 0.11 & 0.08 & 0.07 \\
&$\text{ADF}^{(\GLS)}$ & 0.08 & 0.10 & 0.19 & 0.12 & 0.13 & 0.29 & 0.76 & 0.25 & 0.08 & 0.13 & 0.09 & 0.08 \\
&$\text{ADF}^*$ & 0.04 & 0.04 & 0.07 & 0.04 & 0.04 & 0.06 & 0.44 & 0.06 & 0.04 & 0.05 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.05 & 0.08 & 0.07 & 0.06 & 0.07 & 0.42 & 0.08 & 0.05 & 0.06 & 0.05 & 0.04 \\
&MSB & 0.09 & 0.11 & 0.19 & 0.12 & 0.13 & 0.22 & 0.92 & 0.25 & 0.09 & 0.13 & 0.10 & 0.09 \\
&$\text{MSB}^{(\GLS)*}$ & 0.03 & 0.04 & 0.07 & 0.05 & 0.04 & 0.02 & 0.24 & 0.06 & 0.03 & 0.05 & 0.03 & 0.03 \\
&$\hat{Z}_{\alpha}$ & 0.06 & 0.08 & 0.21 & 0.07 & 0.42 & 1.00 & 1.00 & 0.76 & 0.06 & 0.10 & 0.06 & 0.05 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> Figures/Empirical_Sizes/2022-07-16/Size_table_m_1_T_100_dtype0_BIC.tex <==

\begin{table}[!ht]
\begin{center}
\caption{Size-table-m-1-T-100-dtype0-BIC}
\begin{tabular}{c|cccccccccccc}
\hline
&$\rho_1,\rho_2$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\\hline
&$\text{VR}$ & 0.02 & 0.01 & 0.01 & 0.01 & 0.02 & 0.03 & 0.17 & 0.02 & 0.02 & 0.01 & 0.02 & 0.02 \\
&$\text{VR}^{(\GLS)}$ & 0.02 & 0.01 & 0.01 & 0.01 & 0.02 & 0.03 & 0.17 & 0.02 & 0.02 & 0.01 & 0.02 & 0.02 \\
&ADF & 0.07 & 0.06 & 0.05 & 0.05 & 0.12 & 0.21 & 0.65 & 0.19 & 0.07 & 0.05 & 0.07 & 0.07 \\
&$\text{ADF}^{(\GLS)}$ & 0.07 & 0.06 & 0.05 & 0.05 & 0.12 & 0.21 & 0.65 & 0.19 & 0.07 & 0.05 & 0.07 & 0.07 \\
&$\text{ADF}^*$ & 0.06 & 0.04 & 0.04 & 0.04 & 0.06 & 0.07 & 0.15 & 0.08 & 0.06 & 0.04 & 0.06 & 0.06 \\
&$\text{ADF}^{(\GLS)*}$ & 0.06 & 0.04 & 0.04 & 0.04 & 0.06 & 0.07 & 0.15 & 0.08 & 0.06 & 0.04 & 0.06 & 0.06 \\
&MSB & 0.01 & 0.01 & 0.01 & 0.01 & 0.04 & 0.11 & 0.55 & 0.09 & 0.01 & 0.01 & 0.01 & 0.01 \\
&$\text{MSB}^{(\GLS)*}$ & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.02 & 0.07 & 0.02 & 0.01 & 0.00 & 0.00 & 0.01 \\
&$\hat{Z}_{\alpha}$ & 0.03 & 0.02 & 0.01 & 0.01 & 0.07 & 0.30 & 0.89 & 0.13 & 0.03 & 0.01 & 0.03 & 0.03 \\
&$\text{VR}$ & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.03 & 0.17 & 0.02 & 0.01 & 0.01 & 0.01 & 0.01 \\
&$\text{VR}^{(\GLS)}$ & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.03 & 0.17 & 0.02 & 0.01 & 0.01 & 0.01 & 0.01 \\
&ADF & 0.07 & 0.06 & 0.07 & 0.06 & 0.11 & 0.20 & 0.65 & 0.18 & 0.07 & 0.06 & 0.07 & 0.07 \\
&$\text{ADF}^{(\GLS)}$ & 0.07 & 0.06 & 0.07 & 0.06 & 0.11 & 0.20 & 0.65 & 0.18 & 0.07 & 0.06 & 0.07 & 0.07 \\
&$\text{ADF}^*$ & 0.06 & 0.04 & 0.05 & 0.05 & 0.06 & 0.07 & 0.16 & 0.07 & 0.06 & 0.04 & 0.06 & 0.06 \\
&$\text{ADF}^{(\GLS)*}$ & 0.06 & 0.04 & 0.05 & 0.05 & 0.06 & 0.07 & 0.16 & 0.07 & 0.06 & 0.04 & 0.06 & 0.06 \\
&MSB & 0.01 & 0.01 & 0.02 & 0.02 & 0.04 & 0.11 & 0.56 & 0.08 & 0.01 & 0.01 & 0.01 & 0.01 \\
&$\text{MSB}^{(\GLS)*}$ & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.08 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 \\
&$\hat{Z}_{\alpha}$ & 0.02 & 0.02 & 0.02 & 0.02 & 0.07 & 0.31 & 0.89 & 0.12 & 0.03 & 0.02 & 0.02 & 0.02 \\
&$\text{VR}$ & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.03 & 0.18 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 \\
&$\text{VR}^{(\GLS)}$ & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.03 & 0.18 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 \\
&ADF & 0.06 & 0.08 & 0.11 & 0.08 & 0.11 & 0.22 & 0.67 & 0.18 & 0.06 & 0.08 & 0.07 & 0.06 \\
&$\text{ADF}^{(\GLS)}$ & 0.06 & 0.08 & 0.11 & 0.08 & 0.11 & 0.22 & 0.67 & 0.18 & 0.06 & 0.08 & 0.07 & 0.06 \\
&$\text{ADF}^*$ & 0.05 & 0.05 & 0.07 & 0.06 & 0.06 & 0.07 & 0.18 & 0.07 & 0.06 & 0.06 & 0.06 & 0.06 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.05 & 0.07 & 0.06 & 0.06 & 0.07 & 0.18 & 0.07 & 0.06 & 0.06 & 0.06 & 0.06 \\
&MSB & 0.01 & 0.01 & 0.03 & 0.01 & 0.03 & 0.12 & 0.58 & 0.09 & 0.00 & 0.01 & 0.01 & 0.00 \\
&$\text{MSB}^{(\GLS)*}$ & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.10 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\
&$\hat{Z}_{\alpha}$ & 0.02 & 0.02 & 0.04 & 0.03 & 0.07 & 0.34 & 0.89 & 0.13 & 0.02 & 0.02 & 0.02 & 0.02 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> Figures/Empirical_Sizes/2022-07-16/Size_table_m_1_T_100_dtype1_BIC.tex <==

\begin{table}[!ht]
\begin{center}
\caption{Size-table-m-1-T-100-dtype1-BIC}
\begin{tabular}{c|cccccccccccc}
\hline
&$\rho_1,\rho_2$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\\hline
&$\text{VR}$ & 0.05 & 0.04 & 0.03 & 0.01 & 0.07 & 0.16 & 0.72 & 0.10 & 0.05 & 0.03 & 0.05 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.12 & 0.11 & 0.08 & 0.03 & 0.15 & 0.26 & 0.82 & 0.19 & 0.12 & 0.09 & 0.12 & 0.12 \\
&ADF & 0.06 & 0.05 & 0.04 & 0.03 & 0.19 & 0.39 & 0.97 & 0.35 & 0.06 & 0.03 & 0.07 & 0.06 \\
&$\text{ADF}^{(\GLS)}$ & 0.09 & 0.07 & 0.05 & 0.02 & 0.24 & 0.42 & 0.93 & 0.42 & 0.09 & 0.04 & 0.10 & 0.09 \\
&$\text{ADF}^*$ & 0.04 & 0.01 & 0.02 & 0.02 & 0.06 & 0.07 & 0.36 & 0.09 & 0.04 & 0.01 & 0.05 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.06 & 0.02 & 0.01 & 0.01 & 0.09 & 0.11 & 0.39 & 0.13 & 0.06 & 0.01 & 0.06 & 0.07 \\
&MSB & 0.03 & 0.04 & 0.04 & 0.04 & 0.14 & 0.32 & 0.95 & 0.27 & 0.03 & 0.04 & 0.03 & 0.03 \\
&$\text{MSB}^{(\GLS)*}$ & 0.03 & 0.00 & 0.01 & 0.01 & 0.04 & 0.05 & 0.28 & 0.09 & 0.03 & 0.00 & 0.03 & 0.03 \\
&$\hat{Z}_{\alpha}$ & 0.05 & 0.02 & 0.01 & 0.01 & 0.19 & 0.72 & 1.00 & 0.33 & 0.05 & 0.01 & 0.05 & 0.05 \\
&$\text{VR}$ & 0.05 & 0.04 & 0.03 & 0.01 & 0.07 & 0.19 & 0.78 & 0.11 & 0.05 & 0.03 & 0.05 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.12 & 0.11 & 0.09 & 0.05 & 0.16 & 0.29 & 0.85 & 0.20 & 0.12 & 0.09 & 0.12 & 0.12 \\
&ADF & 0.07 & 0.06 & 0.06 & 0.03 & 0.20 & 0.45 & 0.99 & 0.39 & 0.07 & 0.05 & 0.08 & 0.07 \\
&$\text{ADF}^{(\GLS)}$ & 0.10 & 0.08 & 0.07 & 0.04 & 0.25 & 0.46 & 0.95 & 0.45 & 0.10 & 0.05 & 0.10 & 0.10 \\
&$\text{ADF}^*$ & 0.04 & 0.02 & 0.03 & 0.02 & 0.06 & 0.07 & 0.40 & 0.10 & 0.04 & 0.02 & 0.05 & 0.05 \\
&$\text{ADF}^{(\GLS)*}$ & 0.07 & 0.03 & 0.03 & 0.02 & 0.09 & 0.12 & 0.43 & 0.14 & 0.07 & 0.02 & 0.07 & 0.07 \\
&MSB & 0.03 & 0.05 & 0.05 & 0.04 & 0.15 & 0.38 & 0.98 & 0.32 & 0.03 & 0.04 & 0.03 & 0.03 \\
&$\text{MSB}^{(\GLS)*}$ & 0.03 & 0.01 & 0.02 & 0.02 & 0.04 & 0.06 & 0.31 & 0.09 & 0.03 & 0.01 & 0.03 & 0.03 \\
&$\hat{Z}_{\alpha}$ & 0.06 & 0.03 & 0.03 & 0.02 & 0.21 & 0.79 & 1.00 & 0.39 & 0.06 & 0.02 & 0.06 & 0.06 \\
&$\text{VR}$ & 0.05 & 0.05 & 0.06 & 0.01 & 0.09 & 0.31 & 0.87 & 0.15 & 0.05 & 0.05 & 0.05 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.12 & 0.12 & 0.14 & 0.06 & 0.18 & 0.43 & 0.93 & 0.26 & 0.12 & 0.12 & 0.12 & 0.12 \\
&ADF & 0.07 & 0.10 & 0.17 & 0.05 & 0.24 & 0.65 & 1.00 & 0.53 & 0.07 & 0.10 & 0.08 & 0.07 \\
&$\text{ADF}^{(\GLS)}$ & 0.10 & 0.13 & 0.23 & 0.08 & 0.28 & 0.64 & 0.97 & 0.56 & 0.10 & 0.14 & 0.10 & 0.10 \\
&$\text{ADF}^*$ & 0.04 & 0.04 & 0.08 & 0.03 & 0.06 & 0.11 & 0.47 & 0.11 & 0.04 & 0.05 & 0.05 & 0.05 \\
&$\text{ADF}^{(\GLS)*}$ & 0.07 & 0.06 & 0.12 & 0.05 & 0.09 & 0.15 & 0.50 & 0.16 & 0.07 & 0.08 & 0.07 & 0.07 \\
&MSB & 0.03 & 0.06 & 0.11 & 0.03 & 0.18 & 0.58 & 0.99 & 0.47 & 0.03 & 0.06 & 0.04 & 0.03 \\
&$\text{MSB}^{(\GLS)*}$ & 0.03 & 0.03 & 0.07 & 0.03 & 0.05 & 0.07 & 0.37 & 0.10 & 0.03 & 0.04 & 0.03 & 0.03 \\
&$\hat{Z}_{\alpha}$ & 0.06 & 0.07 & 0.14 & 0.04 & 0.36 & 0.95 & 1.00 & 0.59 & 0.06 & 0.08 & 0.06 & 0.06 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> Figures/Empirical_Sizes/2022-07-16/Size_table_m_1_T_100_dtype2_BIC.tex <==

\begin{table}[!ht]
\begin{center}
\caption{Size-table-m-1-T-100-dtype2-BIC}
\begin{tabular}{c|cccccccccccc}
\hline
&$\rho_1,\rho_2$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\\hline
&$\text{VR}$ & 0.05 & 0.04 & 0.02 & 0.00 & 0.09 & 0.26 & 0.93 & 0.14 & 0.05 & 0.03 & 0.06 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.30 & 0.26 & 0.20 & 0.07 & 0.36 & 0.59 & 0.99 & 0.45 & 0.30 & 0.22 & 0.30 & 0.30 \\
&ADF & 0.07 & 0.06 & 0.05 & 0.02 & 0.28 & 0.55 & 0.99 & 0.50 & 0.07 & 0.03 & 0.07 & 0.07 \\
&$\text{ADF}^{(\GLS)}$ & 0.11 & 0.08 & 0.07 & 0.03 & 0.33 & 0.57 & 0.98 & 0.56 & 0.11 & 0.05 & 0.11 & 0.11 \\
&$\text{ADF}^*$ & 0.04 & 0.01 & 0.00 & 0.01 & 0.06 & 0.10 & 0.52 & 0.12 & 0.04 & 0.00 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.06 & 0.01 & 0.01 & 0.01 & 0.09 & 0.13 & 0.55 & 0.17 & 0.06 & 0.00 & 0.07 & 0.06 \\
&MSB & 0.03 & 0.06 & 0.07 & 0.07 & 0.14 & 0.42 & 0.98 & 0.29 & 0.03 & 0.05 & 0.03 & 0.03 \\
&$\text{MSB}^{(\GLS)*}$ & 0.01 & 0.00 & 0.01 & 0.02 & 0.04 & 0.07 & 0.43 & 0.10 & 0.01 & 0.00 & 0.02 & 0.02 \\
&$\hat{Z}_{\alpha}$ & 0.04 & 0.01 & 0.00 & 0.00 & 0.24 & 0.87 & 1.00 & 0.43 & 0.04 & 0.00 & 0.05 & 0.04 \\
&$\text{VR}$ & 0.05 & 0.04 & 0.03 & 0.00 & 0.09 & 0.30 & 0.94 & 0.15 & 0.05 & 0.03 & 0.05 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.30 & 0.26 & 0.22 & 0.08 & 0.38 & 0.64 & 0.99 & 0.47 & 0.30 & 0.23 & 0.30 & 0.30 \\
&ADF & 0.07 & 0.06 & 0.05 & 0.03 & 0.30 & 0.63 & 1.00 & 0.55 & 0.07 & 0.04 & 0.08 & 0.08 \\
&$\text{ADF}^{(\GLS)}$ & 0.10 & 0.08 & 0.07 & 0.03 & 0.34 & 0.63 & 0.99 & 0.60 & 0.10 & 0.06 & 0.10 & 0.10 \\
&$\text{ADF}^*$ & 0.04 & 0.01 & 0.01 & 0.01 & 0.06 & 0.11 & 0.50 & 0.12 & 0.04 & 0.01 & 0.05 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.06 & 0.02 & 0.01 & 0.01 & 0.09 & 0.14 & 0.52 & 0.18 & 0.06 & 0.01 & 0.06 & 0.06 \\
&MSB & 0.02 & 0.05 & 0.05 & 0.06 & 0.16 & 0.47 & 0.99 & 0.34 & 0.02 & 0.04 & 0.03 & 0.02 \\
&$\text{MSB}^{(\GLS)*}$ & 0.02 & 0.00 & 0.01 & 0.02 & 0.04 & 0.07 & 0.40 & 0.10 & 0.02 & 0.00 & 0.02 & 0.02 \\
&$\hat{Z}_{\alpha}$ & 0.04 & 0.01 & 0.01 & 0.00 & 0.28 & 0.93 & 1.00 & 0.48 & 0.04 & 0.01 & 0.05 & 0.05 \\
&$\text{VR}$ & 0.05 & 0.05 & 0.06 & 0.00 & 0.11 & 0.48 & 0.98 & 0.20 & 0.05 & 0.04 & 0.05 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.29 & 0.29 & 0.32 & 0.09 & 0.43 & 0.81 & 1.00 & 0.56 & 0.29 & 0.28 & 0.30 & 0.29 \\
&ADF & 0.07 & 0.10 & 0.14 & 0.02 & 0.36 & 0.82 & 1.00 & 0.70 & 0.07 & 0.08 & 0.08 & 0.08 \\
&$\text{ADF}^{(\GLS)}$ & 0.10 & 0.13 & 0.20 & 0.03 & 0.38 & 0.80 & 0.99 & 0.72 & 0.10 & 0.12 & 0.11 & 0.10 \\
&$\text{ADF}^*$ & 0.04 & 0.03 & 0.06 & 0.01 & 0.07 & 0.15 & 0.47 & 0.16 & 0.04 & 0.03 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.06 & 0.05 & 0.09 & 0.01 & 0.10 & 0.19 & 0.50 & 0.20 & 0.06 & 0.06 & 0.06 & 0.06 \\
&MSB & 0.02 & 0.04 & 0.06 & 0.03 & 0.23 & 0.70 & 0.99 & 0.54 & 0.02 & 0.04 & 0.03 & 0.02 \\
&$\text{MSB}^{(\GLS)*}$ & 0.02 & 0.01 & 0.03 & 0.01 & 0.04 & 0.10 & 0.37 & 0.13 & 0.02 & 0.01 & 0.02 & 0.02 \\
&$\hat{Z}_{\alpha}$ & 0.05 & 0.05 & 0.09 & 0.00 & 0.46 & 1.00 & 1.00 & 0.70 & 0.05 & 0.05 & 0.05 & 0.05 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> Figures/Empirical_Sizes/2022-07-16/Size_table_m_1_T_250_dtype0_BIC.tex <==

\begin{table}[!ht]
\begin{center}
\caption{Size-table-m-1-T-250-dtype0-BIC}
\begin{tabular}{c|cccccccccccc}
\hline
&$\rho_1,\rho_2$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\\hline
&$\text{VR}$ & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 & 0.03 & 0.14 & 0.03 & 0.02 & 0.02 & 0.02 & 0.02 \\
&$\text{VR}^{(\GLS)}$ & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 & 0.03 & 0.14 & 0.03 & 0.02 & 0.02 & 0.02 & 0.02 \\
&ADF & 0.05 & 0.05 & 0.04 & 0.03 & 0.09 & 0.16 & 0.58 & 0.16 & 0.06 & 0.04 & 0.06 & 0.05 \\
&$\text{ADF}^{(\GLS)}$ & 0.05 & 0.05 & 0.04 & 0.03 & 0.09 & 0.16 & 0.58 & 0.16 & 0.06 & 0.04 & 0.06 & 0.05 \\
&$\text{ADF}^*$ & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.06 & 0.12 & 0.07 & 0.05 & 0.03 & 0.05 & 0.05 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.03 & 0.03 & 0.03 & 0.05 & 0.06 & 0.12 & 0.07 & 0.05 & 0.03 & 0.05 & 0.05 \\
&MSB & 0.02 & 0.02 & 0.01 & 0.01 & 0.04 & 0.09 & 0.45 & 0.11 & 0.02 & 0.01 & 0.02 & 0.02 \\
&$\text{MSB}^{(\GLS)*}$ & 0.02 & 0.01 & 0.01 & 0.01 & 0.02 & 0.02 & 0.02 & 0.03 & 0.01 & 0.00 & 0.02 & 0.01 \\
&$\hat{Z}_{\alpha}$ & 0.03 & 0.02 & 0.02 & 0.01 & 0.07 & 0.31 & 0.94 & 0.14 & 0.03 & 0.02 & 0.03 & 0.03 \\
&$\text{VR}$ & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 & 0.03 & 0.16 & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 \\
&$\text{VR}^{(\GLS)}$ & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 & 0.03 & 0.16 & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 \\
&ADF & 0.05 & 0.05 & 0.06 & 0.05 & 0.08 & 0.17 & 0.62 & 0.15 & 0.05 & 0.05 & 0.06 & 0.06 \\
&$\text{ADF}^{(\GLS)}$ & 0.05 & 0.05 & 0.06 & 0.05 & 0.08 & 0.17 & 0.62 & 0.15 & 0.05 & 0.05 & 0.06 & 0.06 \\
&$\text{ADF}^*$ & 0.05 & 0.04 & 0.05 & 0.04 & 0.05 & 0.07 & 0.15 & 0.06 & 0.05 & 0.04 & 0.05 & 0.05 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.04 & 0.05 & 0.04 & 0.05 & 0.07 & 0.15 & 0.06 & 0.05 & 0.04 & 0.05 & 0.05 \\
&MSB & 0.02 & 0.02 & 0.02 & 0.02 & 0.04 & 0.09 & 0.49 & 0.09 & 0.02 & 0.02 & 0.02 & 0.02 \\
&$\text{MSB}^{(\GLS)*}$ & 0.01 & 0.01 & 0.01 & 0.01 & 0.02 & 0.01 & 0.02 & 0.02 & 0.01 & 0.01 & 0.01 & 0.01 \\
&$\hat{Z}_{\alpha}$ & 0.03 & 0.02 & 0.02 & 0.03 & 0.07 & 0.35 & 0.95 & 0.15 & 0.03 & 0.02 & 0.03 & 0.03 \\
&$\text{VR}$ & 0.01 & 0.01 & 0.01 & 0.02 & 0.02 & 0.03 & 0.18 & 0.02 & 0.01 & 0.01 & 0.01 & 0.01 \\
&$\text{VR}^{(\GLS)}$ & 0.01 & 0.01 & 0.01 & 0.02 & 0.02 & 0.03 & 0.18 & 0.02 & 0.01 & 0.01 & 0.01 & 0.01 \\
&ADF & 0.06 & 0.07 & 0.13 & 0.13 & 0.09 & 0.20 & 0.67 & 0.16 & 0.06 & 0.09 & 0.06 & 0.06 \\
&$\text{ADF}^{(\GLS)}$ & 0.06 & 0.07 & 0.13 & 0.13 & 0.09 & 0.20 & 0.67 & 0.16 & 0.06 & 0.09 & 0.06 & 0.06 \\
&$\text{ADF}^*$ & 0.05 & 0.05 & 0.08 & 0.11 & 0.05 & 0.07 & 0.21 & 0.07 & 0.05 & 0.06 & 0.05 & 0.05 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.05 & 0.08 & 0.11 & 0.05 & 0.07 & 0.21 & 0.07 & 0.05 & 0.06 & 0.05 & 0.05 \\
&MSB & 0.01 & 0.03 & 0.07 & 0.07 & 0.03 & 0.10 & 0.55 & 0.09 & 0.01 & 0.03 & 0.01 & 0.01 \\
&$\text{MSB}^{(\GLS)*}$ & 0.01 & 0.01 & 0.03 & 0.05 & 0.01 & 0.01 & 0.05 & 0.01 & 0.01 & 0.02 & 0.01 & 0.01 \\
&$\hat{Z}_{\alpha}$ & 0.02 & 0.03 & 0.08 & 0.09 & 0.08 & 0.43 & 0.96 & 0.18 & 0.02 & 0.04 & 0.03 & 0.02 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> Figures/Empirical_Sizes/2022-07-16/Size_table_m_1_T_250_dtype1_BIC.tex <==

\begin{table}[!ht]
\begin{center}
\caption{Size-table-m-1-T-250-dtype1-BIC}
\begin{tabular}{c|cccccccccccc}
\hline
&$\rho_1,\rho_2$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\\hline
&$\text{VR}$ & 0.05 & 0.05 & 0.04 & 0.02 & 0.06 & 0.10 & 0.56 & 0.08 & 0.05 & 0.04 & 0.06 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.10 & 0.10 & 0.09 & 0.06 & 0.11 & 0.15 & 0.55 & 0.12 & 0.10 & 0.09 & 0.10 & 0.10 \\
&ADF & 0.05 & 0.04 & 0.03 & 0.02 & 0.10 & 0.22 & 0.89 & 0.23 & 0.05 & 0.03 & 0.05 & 0.05 \\
&$\text{ADF}^{(\GLS)}$ & 0.06 & 0.05 & 0.04 & 0.02 & 0.11 & 0.22 & 0.76 & 0.23 & 0.06 & 0.03 & 0.06 & 0.06 \\
&$\text{ADF}^*$ & 0.04 & 0.01 & 0.02 & 0.01 & 0.05 & 0.05 & 0.17 & 0.06 & 0.04 & 0.01 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.04 & 0.01 & 0.02 & 0.01 & 0.06 & 0.07 & 0.17 & 0.08 & 0.04 & 0.01 & 0.05 & 0.05 \\
&MSB & 0.04 & 0.05 & 0.04 & 0.03 & 0.09 & 0.20 & 0.84 & 0.24 & 0.04 & 0.03 & 0.04 & 0.04 \\
&$\text{MSB}^{(\GLS)*}$ & 0.03 & 0.01 & 0.02 & 0.01 & 0.05 & 0.03 & 0.04 & 0.06 & 0.03 & 0.01 & 0.04 & 0.03 \\
&$\hat{Z}_{\alpha}$ & 0.06 & 0.03 & 0.02 & 0.00 & 0.15 & 0.64 & 1.00 & 0.31 & 0.06 & 0.02 & 0.06 & 0.06 \\
&$\text{VR}$ & 0.05 & 0.05 & 0.05 & 0.03 & 0.06 & 0.12 & 0.66 & 0.08 & 0.05 & 0.05 & 0.06 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.10 & 0.10 & 0.10 & 0.07 & 0.12 & 0.17 & 0.62 & 0.13 & 0.10 & 0.10 & 0.11 & 0.10 \\
&ADF & 0.05 & 0.05 & 0.05 & 0.04 & 0.11 & 0.27 & 0.95 & 0.26 & 0.05 & 0.04 & 0.06 & 0.05 \\
&$\text{ADF}^{(\GLS)}$ & 0.06 & 0.06 & 0.06 & 0.04 & 0.12 & 0.26 & 0.81 & 0.25 & 0.06 & 0.04 & 0.07 & 0.06 \\
&$\text{ADF}^*$ & 0.04 & 0.02 & 0.03 & 0.03 & 0.05 & 0.06 & 0.23 & 0.06 & 0.04 & 0.02 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.03 & 0.04 & 0.03 & 0.06 & 0.08 & 0.23 & 0.08 & 0.05 & 0.02 & 0.05 & 0.05 \\
&MSB & 0.04 & 0.05 & 0.05 & 0.03 & 0.10 & 0.24 & 0.91 & 0.26 & 0.04 & 0.03 & 0.05 & 0.05 \\
&$\text{MSB}^{(\GLS)*}$ & 0.04 & 0.02 & 0.04 & 0.03 & 0.05 & 0.03 & 0.08 & 0.06 & 0.04 & 0.02 & 0.04 & 0.04 \\
&$\hat{Z}_{\alpha}$ & 0.06 & 0.04 & 0.04 & 0.03 & 0.18 & 0.74 & 1.00 & 0.36 & 0.06 & 0.03 & 0.06 & 0.06 \\
&$\text{VR}$ & 0.05 & 0.05 & 0.06 & 0.06 & 0.07 & 0.19 & 0.83 & 0.10 & 0.05 & 0.06 & 0.06 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.10 & 0.10 & 0.11 & 0.12 & 0.12 & 0.25 & 0.74 & 0.15 & 0.10 & 0.10 & 0.10 & 0.10 \\
&ADF & 0.05 & 0.09 & 0.20 & 0.13 & 0.14 & 0.43 & 0.99 & 0.34 & 0.05 & 0.10 & 0.06 & 0.05 \\
&$\text{ADF}^{(\GLS)}$ & 0.06 & 0.10 & 0.22 & 0.18 & 0.15 & 0.39 & 0.89 & 0.32 & 0.06 & 0.13 & 0.07 & 0.06 \\
&$\text{ADF}^*$ & 0.04 & 0.04 & 0.07 & 0.10 & 0.05 & 0.06 & 0.41 & 0.07 & 0.04 & 0.05 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.05 & 0.10 & 0.15 & 0.07 & 0.08 & 0.39 & 0.09 & 0.05 & 0.07 & 0.05 & 0.05 \\
&MSB & 0.04 & 0.08 & 0.21 & 0.14 & 0.13 & 0.37 & 0.99 & 0.34 & 0.04 & 0.10 & 0.05 & 0.04 \\
&$\text{MSB}^{(\GLS)*}$ & 0.04 & 0.04 & 0.09 & 0.13 & 0.05 & 0.02 & 0.18 & 0.07 & 0.04 & 0.05 & 0.04 & 0.04 \\
&$\hat{Z}_{\alpha}$ & 0.06 & 0.08 & 0.19 & 0.16 & 0.29 & 0.94 & 1.00 & 0.57 & 0.06 & 0.10 & 0.06 & 0.06 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> Figures/Empirical_Sizes/2022-07-16/Size_table_m_1_T_250_dtype2_BIC.tex <==

\begin{table}[!ht]
\begin{center}
\caption{Size-table-m-1-T-250-dtype2-BIC}
\begin{tabular}{c|cccccccccccc}
\hline
&$\rho_1,\rho_2$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\\hline
&$\text{VR}$ & 0.05 & 0.05 & 0.03 & 0.01 & 0.07 & 0.15 & 0.83 & 0.10 & 0.05 & 0.04 & 0.06 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.13 & 0.12 & 0.11 & 0.05 & 0.15 & 0.23 & 0.65 & 0.18 & 0.13 & 0.11 & 0.14 & 0.13 \\
&ADF & 0.05 & 0.05 & 0.04 & 0.02 & 0.13 & 0.34 & 0.98 & 0.34 & 0.05 & 0.03 & 0.06 & 0.06 \\
&$\text{ADF}^{(\GLS)}$ & 0.07 & 0.07 & 0.05 & 0.02 & 0.15 & 0.33 & 0.91 & 0.34 & 0.07 & 0.03 & 0.07 & 0.07 \\
&$\text{ADF}^*$ & 0.04 & 0.01 & 0.02 & 0.01 & 0.05 & 0.06 & 0.25 & 0.07 & 0.04 & 0.00 & 0.04 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.01 & 0.02 & 0.01 & 0.07 & 0.08 & 0.25 & 0.09 & 0.05 & 0.00 & 0.05 & 0.05 \\
&MSB & 0.03 & 0.05 & 0.05 & 0.03 & 0.11 & 0.27 & 0.96 & 0.31 & 0.03 & 0.04 & 0.04 & 0.03 \\
&$\text{MSB}^{(\GLS)*}$ & 0.03 & 0.00 & 0.03 & 0.01 & 0.05 & 0.04 & 0.11 & 0.07 & 0.03 & 0.00 & 0.03 & 0.03 \\
&$\hat{Z}_{\alpha}$ & 0.05 & 0.03 & 0.01 & 0.00 & 0.21 & 0.83 & 1.00 & 0.43 & 0.05 & 0.01 & 0.06 & 0.06 \\
&$\text{VR}$ & 0.05 & 0.05 & 0.04 & 0.01 & 0.07 & 0.19 & 0.91 & 0.10 & 0.05 & 0.04 & 0.05 & 0.05 \\
&$\text{VR}^{(\GLS)}$ & 0.13 & 0.12 & 0.11 & 0.07 & 0.15 & 0.25 & 0.69 & 0.19 & 0.13 & 0.11 & 0.13 & 0.13 \\
&ADF & 0.06 & 0.06 & 0.05 & 0.03 & 0.14 & 0.40 & 0.99 & 0.38 & 0.06 & 0.04 & 0.07 & 0.06 \\
&$\text{ADF}^{(\GLS)}$ & 0.07 & 0.06 & 0.05 & 0.03 & 0.16 & 0.39 & 0.94 & 0.37 & 0.07 & 0.04 & 0.07 & 0.07 \\
&$\text{ADF}^*$ & 0.05 & 0.02 & 0.02 & 0.02 & 0.05 & 0.06 & 0.31 & 0.07 & 0.05 & 0.01 & 0.05 & 0.05 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.02 & 0.03 & 0.02 & 0.06 & 0.07 & 0.30 & 0.09 & 0.05 & 0.01 & 0.05 & 0.05 \\
&MSB & 0.03 & 0.05 & 0.04 & 0.03 & 0.11 & 0.32 & 0.98 & 0.35 & 0.03 & 0.03 & 0.04 & 0.04 \\
&$\text{MSB}^{(\GLS)*}$ & 0.03 & 0.01 & 0.02 & 0.02 & 0.05 & 0.03 & 0.15 & 0.07 & 0.03 & 0.01 & 0.04 & 0.03 \\
&$\hat{Z}_{\alpha}$ & 0.06 & 0.03 & 0.03 & 0.01 & 0.25 & 0.91 & 1.00 & 0.51 & 0.06 & 0.02 & 0.06 & 0.06 \\
&$\text{VR}$ & 0.05 & 0.06 & 0.07 & 0.03 & 0.09 & 0.32 & 0.99 & 0.15 & 0.05 & 0.06 & 0.05 & 0.06 \\
&$\text{VR}^{(\GLS)}$ & 0.13 & 0.13 & 0.15 & 0.13 & 0.16 & 0.35 & 0.73 & 0.22 & 0.13 & 0.13 & 0.13 & 0.13 \\
&ADF & 0.06 & 0.10 & 0.24 & 0.08 & 0.19 & 0.61 & 1.00 & 0.49 & 0.06 & 0.12 & 0.07 & 0.06 \\
&$\text{ADF}^{(\GLS)}$ & 0.07 & 0.11 & 0.27 & 0.11 & 0.20 & 0.57 & 0.96 & 0.48 & 0.07 & 0.14 & 0.08 & 0.07 \\
&$\text{ADF}^*$ & 0.04 & 0.04 & 0.08 & 0.05 & 0.05 & 0.07 & 0.45 & 0.08 & 0.04 & 0.05 & 0.05 & 0.04 \\
&$\text{ADF}^{(\GLS)*}$ & 0.05 & 0.05 & 0.10 & 0.08 & 0.07 & 0.09 & 0.43 & 0.10 & 0.05 & 0.07 & 0.05 & 0.05 \\
&MSB & 0.04 & 0.07 & 0.21 & 0.06 & 0.15 & 0.49 & 1.00 & 0.46 & 0.04 & 0.09 & 0.04 & 0.04 \\
&$\text{MSB}^{(\GLS)*}$ & 0.03 & 0.04 & 0.08 & 0.06 & 0.05 & 0.03 & 0.25 & 0.07 & 0.03 & 0.05 & 0.04 & 0.04 \\
&$\hat{Z}_{\alpha}$ & 0.06 & 0.08 & 0.21 & 0.07 & 0.42 & 1.00 & 1.00 & 0.76 & 0.06 & 0.10 & 0.06 & 0.05 \\
\hline
\end{tabular}
\end{center}
\end{table}

